Data Augmentation vs. Equivariant Networks: A Theory of Generalization on Dynamics Forecasting

Exploiting symmetry in dynamical systems is a powerful way to improve the generalization of deep learning. The model learns to be invariant to transformation and hence is more robust to distribution shift. Data augmentation and equivariant networks are two major approaches to injecting symmetry into learning. However, their exact role in improving generalization is not well understood. In this work, we derive the generalization bounds for data augmentation and equivariant networks, characterizing their effect on learning in a unified framework. Unlike most prior theories for the i.i.d. setting, we focus on non-stationary dynamics forecasting with complex temporal dependencies.

==> sections/checklist.tex <==
%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}


==> sections/general_framework/sym_intro.tex <==


In this subsection, we give the formal definitions of data augmentation, equivariance and approximate equivariance in our deterministic dynamics forecasting setting.

\subsection{Data Aug. Introduces Symmetry.}
Consider a finite group $G$ that acts on the observed time series, we assume that for any $g \in G$, there is a certain amount of symmetry in the distribution, that is $Z_t^{(i)} \approx_d g Z_t^{(i)}, Z_t^{(i)} \sim \mathbb{P}$. We assume the group transformations are norm-preserving, i.e. $\|g\| = 1 \; \forall g \in G$, such as rotation and translation.


\begin{definition}[Data Augmentation]
Given a finite group $G$, we assume the augmented samples are the original samples applied with transformations uniformly sampled from the group. In other words, for every sample $Z_t^{(i)}$ in the original training set, we augment $\{gZ_t^{(i)}, g\in G\}$. Then the augmented training set is the $|G|$ times bigger than the original training set. 
\end{definition}



\subsection{Equivariant Networks are Symmetry-Aware}
\begin{definition}[Approximate Equivariance]\label{def_app}
Let $f \colon X \to Y$ be a function and $G$ be a group. Assume that $G$ acts on $X$ and $Y$ via representations $\rho_{\text{in}}$ and $\rho_{\text{out}}$. We say $f$ is $\epsilon$-approximately $G$-equivariant if for any $g \in G$, 
$$
    \|f(\rho_{\text{in}}(g)(x)) - \rho_{\text{out}}(g)f(x)\| \leq \epsilon.
$$
\end{definition}
Note that strictly equivariant functions are $\epsilon = 0$ approximately equivariant. Recently, some works have explored the idea of building approximately equivariant models \cite{wang2022approximately, finzi2021residual}. In our paper, we assume these approximately equivariant models can learn the correct amount of equivariance in the data.

We define equivariance error, which quantifies for which $\epsilon$ the function $f$ is $\epsilon$-approximate equivariant.

\begin{definition}[Equivariance Error]
Let $f \colon X \to Y$ be a function and $G$ be a group. Assume that $G$ acts on $X$ and $Y$ via representation $\rho_{\text{in}}$ and $\rho_{\text{out}}$. Then the \textbf{equivariance error} of $f$ is 
$$
\|f\|_{EE} = \sup_{x,g}
%\frac{
\|f(\rho_{\text{in}}(g)(x)) - \rho_{\text{out}}(g)f(x)\|.
%}{\|x\|\|g\|}
$$
\end{definition}

That is, $f$ is $\epsilon$-approximately equivariant if and only if $\| f\|_\mathrm{EE} < \epsilon.$ 

==> sections/iid.tex <==
% \begin{theorem}\label{thm:equ-approx}
% Let $L(\theta, \cdot)$ be Lipschitz uniformly over $\theta$, with a Lipschitz constant $\|L\|_{\text{Lip}}$ and $\xi$ be the data equivariance error. Then with probability at least $1-\delta$ over the draw of $(X_1, Y_1), ..., (X_n, Y_n) \in \mathcal{X}$, we have 
% {\setlength{\mathindent}{0cm}
% \begin{equation}
% \begin{aligned}
% \resizebox{.99\hsize}{!}{
% $\mathbb{E}L(\hat{\theta}_G, \{X, Y\}) - \mathbb{E}L(\theta^*, \{X, Y\}) \leq 2 \mathcal{R}(\bar{L}\circ \Theta) + \sqrt{\frac{2 \log (2/\sigma)}{n}} + 2\|L\|_{\text{Lip}}\cdot\mathbb{E}_G \mathcal{W}(\{X, Y\}, \{g X, g Y\})$}\nonumber
% \end{aligned}
% \end{equation}
% }
% {\setlength{\mathindent}{0cm}
% \begin{equation}
% \begin{aligned}
% \resizebox{.99\hsize}{!}{
% $\mathbb{E}L(\hat{\theta}_E, \{X, Y\}) - \mathbb{E}L(\theta^*, \{X, Y\}) \leq 2 \mathcal{R}(L\circ \Theta_E) + \sqrt{\frac{2 \log (2/\sigma)}{n}} + \|L\|_{\text{Lip}}\cdot\mathbb{E}_G \mathcal{W}(\{X, Y\}, \{g X, g Y\})$}\nonumber
% \end{aligned}
% \end{equation}
% }
% {\setlength{\mathindent}{0cm}
% \begin{equation}
% \begin{aligned}
% \resizebox{.99\hsize}{!}{
% $\mathbb{E}L(\hat{\theta}_{AE}, \{X, Y\}) - \mathbb{E}L(\theta^*, \{X, Y\}) \leq 2 \mathcal{R}(L\circ \Theta_{AE}) + \sqrt{\frac{2 \log (2/\sigma)}{n}} + \|L\|_{\text{Lip}}\cdot\mathbb{E}_G \mathcal{W}(\{X, Y\}, \{g X, g Y\})- \|\hat{\theta}_{AE}\|_{EE} + 2\xi$}\nonumber
% \end{aligned}
% \end{equation}
% }

% \end{theorem}

==> sections/relate.tex <==
Developing neural nets that preserve symmetries has been a fundamental task in deep learning. There have been a lot of work in developing efficient data augmentation techniques that enable neural nets to be invariant to symmetry transformations and noise \cite{hernandez2018data, dao2019kernel, hernandez2018further, rajput2019does, ratner2017learning, zhou2022do}. In addition, incorporating symmetry into deep neural nets to design equivariant DL models have also achieved remarkable success in learning image data \cite{worrall2019deep, cohen2019gauge, cohen2016steerable, weiler2019e2cnn, cohen2018spherical} and physical dynamics \cite{wang2021incorporating, wang2022approximately, ling2016ra, shi2021learning}. 


However, real world dynamics rarely conforms to the strict mathematical symmetry. A perfectly equivariant model may have trouble learning partial or approximated symmetries in the real-world data. Thus, a few works recently explored the idea of building approximately equivariant models and empirically demonstrated the benefits of it in modeling real-world data.  \cite{van2022relaxing, romero2021learning}. For example, \cite{finzi2021residual} proposed the soft equivariant layer by directly summing up a flexible layer with one that has strong equivariance inductive biases to model the soft equivariance. \cite{wang2022approximately} design approximately equivariant models by relaxing the weight sharing schemes in the equivariant convolutional layers. 


